Metatickles and Death in Damascus

The prescriptions of our two most prominent strands of decision theory, evidential and causal, differ in a general class of problems known as Newcomb problems. In these, evidential decision theory prescribes choosing a dominated act. Attempts have been made at reconciling the two theories by relying on additional requirements such as ratification (Jeffrey 1983) or "tickles" (Eells 1982). It has been argued that such attempts have failed (Lewis 1981a; Skyrms 1982). More recently, Huttegger (forthcoming) has developed a version of deliberative decision theory that reconciles the prescriptions of the evidentialist and causalist. In this paper, I extend this framework to problems characterised by decision instability, and show that it cannot deliver a resolute answer under a plausible specification of the tickle. I prove that there exists a robust method of determining whether the specification of the tickle matters for all two-state, two-act problems whose payoff tables exhibit some basic mathematical relationships. One upshot is that we have a principled way of knowing ex-ante whether a reconciliation of evidential and causal decision theory is plausible for a wide range of decision problems under this framework. Another upshot is that the tickle approach needs further work to achieve full reconciliation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{359}
\providecommand{\publicationstatus}{This is a revision of a paper with the same title,\\
published in EPTCS 379, 2023, pp.\ 359--378,\\
doi:\href{http://dx.doi.org/10.4204/EPTCS.379.29}{10.4204/EPTCS.379.29}}
\pdfoutput=1

